Does Manipulating Tokenization Aid Cross-Lingual Transfer? A Study on POS Tagging for Non-Standardized Languages

One of the challenges with finetuning pretrained language models (PLMs) is that their tokenizer is optimized for the language(s) it was pretrained on, but brittle when it comes to previously unseen variations in the data. This can for instance be observed when finetuning PLMs on one language and evaluating them on data in a closely related language variety with no standardized orthography. Despite the high linguistic similarity, tokenization no longer corresponds to meaningful representations of the target data, leading to low performance in, e.g., part-of-speech tagging. In this work, we finetune PLMs on seven languages from three different families and analyze their zero-shot performance on closely related, non-standardized varieties. We consider different measures for the divergence in the tokenization of the source and target data, and the way they can be adjusted by manipulating the tokenization during the finetuning step. Overall, we find that the similarity between the percentage of words that get split into subwords in the source and target data (the split word ratio difference) is the strongest predictor for model performance on target data.

==> tables/accuracies.tex <==
\begin{tabular}
{l@{\hspace{3mm}}l
*{6}{S[table-format=2.0]}
@{}p{4.6mm}@{}
*{6}{S[table-format=2.0]}
@{}p{4.6mm}@{}
*{6}{S[table-format=2.0]}}
\toprule
Source & Target & \multicolumn{6}{c}{Monolingual PLM} && \multicolumn{6}{c}{mBERT} && \multicolumn{6}{c}{XLM-R} \\ 
\cmidrule(lr){3-8} \cmidrule(lr){10-15} \cmidrule(lr){17-22}
 & \multicolumn{1}{r}{Noise:} & 0 & 15 & 35 & 55 & 75 & 95 && 0 & 15 & 35 & 55 & 75 & 95 && 0 & 15 & 35 & 55 & 75 & 95 \\
 \midrule
German & Alsatian G. & \cellcolor[HTML]{EBDAA6}44 & \cellcolor[HTML]{BBA17E}71 & \cellcolor[HTML]{AD9385}\color{white} 76 & \cellcolor[HTML]{A98F87}\color{white} 77 & \cellcolor[HTML]{A88D88}\color{white} \bestval{78} & \cellcolor[HTML]{AA9087}\color{white} 77 &&
\cellcolor[HTML]{DEC473}58 & \cellcolor[HTML]{AD9385}\color{white} 76 & \cellcolor[HTML]{A88E87}\color{white} 78 & \cellcolor[HTML]{A78D88}\color{white} \bestval{78} & \cellcolor[HTML]{A98F87}\color{white} 77 & \cellcolor[HTML]{AB9186}\color{white} 76 &&
\cellcolor[HTML]{E9D79F}46 & \cellcolor[HTML]{BDA37D}71 & \cellcolor[HTML]{AB9186}\color{white} 76 & \cellcolor[HTML]{A78D88}\color{white} \bestval{78} & \cellcolor[HTML]{A98F87}\color{white} 77 & \cellcolor[HTML]{AA9086}\color{white} 77 \\
German & Swiss German & \cellcolor[HTML]{E1CA7F}55 & \cellcolor[HTML]{A68C88}\color{white} 78 & \cellcolor[HTML]{A1878B}\color{white} \bestval{80} & \cellcolor[HTML]{A1878B}\color{white} 80 & \cellcolor[HTML]{A2888A}\color{white} 79 & \cellcolor[HTML]{A58B89}\color{white} 78 && 
\cellcolor[HTML]{D5BA71}62 & \cellcolor[HTML]{A78D88}\color{white} 78 & \cellcolor[HTML]{A58B89}\color{white} 78 & \cellcolor[HTML]{A58B89}\color{white} \bestval{79} & \cellcolor[HTML]{A68C88}\color{white} 78 & \cellcolor[HTML]{AA8F87}\color{white} 77 &&
\cellcolor[HTML]{E0C87B}56 & \cellcolor[HTML]{AB9186}\color{white} 77 & \cellcolor[HTML]{A3898A}\color{white} 79 & \cellcolor[HTML]{A3898A}\color{white} \bestval{79} & \cellcolor[HTML]{A3898A}\color{white} 79 & \cellcolor[HTML]{A68C88}\color{white} 78 \\
\itshape German & \itshape German & \cellcolor[HTML]{6A51A5}\color{white} \itbestval{98} & \cellcolor[HTML]{6A51A5}\color{white} \itcell{98} & \cellcolor[HTML]{6A51A5}\color{white} \itcell{98} & \cellcolor[HTML]{6A51A5}\color{white} \itcell{98} & \cellcolor[HTML]{6A51A5}\color{white} \itcell{98} & \cellcolor[HTML]{6C53A4}\color{white} \itcell{98} && 
\cellcolor[HTML]{6A51A5}\color{white} \itbestval{98} & \cellcolor[HTML]{6A51A5}\color{white} \itcell{98} & \cellcolor[HTML]{6A51A5}\color{white} \itcell{98} & \cellcolor[HTML]{6A51A5}\color{white} \itcell{98} & \cellcolor[HTML]{6A51A5}\color{white} \itcell{98} & \cellcolor[HTML]{6B52A5}\color{white} \itcell{98} &&
\cellcolor[HTML]{6A51A5}\color{white} \itbestval{98} & \cellcolor[HTML]{6A51A5}\color{white} \itcell{98} & \cellcolor[HTML]{6A51A5}\color{white} \itcell{98} & \cellcolor[HTML]{6A51A5}\color{white} \itcell{98} & \cellcolor[HTML]{6A51A5}\color{white} \itcell{98} & \cellcolor[HTML]{6B52A5}\color{white} \itcell{98} \\
\\[\spacer]
German & Low Saxon* & \cellcolor[HTML]{FFFFFF}18 & \cellcolor[HTML]{F1E6C3}35 & \cellcolor[HTML]{E7D396}48 & \cellcolor[HTML]{E5CF8D}51 & \cellcolor[HTML]{DFC574}58 & \cellcolor[HTML]{DCC16E} \bestval{60} && 
\cellcolor[HTML]{F1E5C0}36 & \cellcolor[HTML]{DBC06F}61 & \cellcolor[HTML]{CCB176}66 & \cellcolor[HTML]{C5AB79}\bestval{68} & \cellcolor[HTML]{C8AE78}67 & \cellcolor[HTML]{C9AE78}67 && 
\cellcolor[HTML]{F9F4E3}26 & \cellcolor[HTML]{EAD9A4}44 & \cellcolor[HTML]{DFC574}58 & \cellcolor[HTML]{BBA17E}71 & \cellcolor[HTML]{BBA07E}\bestval{71} & \cellcolor[HTML]{BCA27E}71 \\
Dutch & Low Saxon* & \cellcolor[HTML]{E4CD88}52 & \cellcolor[HTML]{D6BB71}62 & \cellcolor[HTML]{D2B873}63 & \cellcolor[HTML]{D0B574}\bestval{64} & \cellcolor[HTML]{D1B674}64 & \cellcolor[HTML]{D4BA72}63 && 
\cellcolor[HTML]{B69B81}73 & \cellcolor[HTML]{B19783}\color{white} 75 & \cellcolor[HTML]{AF9584}\color{white} \bestval{75} & \cellcolor[HTML]{B09683}\color{white} 75 & \cellcolor[HTML]{B59A81}73 & \cellcolor[HTML]{BAA07F}72 && 
\cellcolor[HTML]{D2B773}63 & \cellcolor[HTML]{BDA27D}71 & \cellcolor[HTML]{B59B81}73 & \cellcolor[HTML]{B59B81}\bestval{73} & \cellcolor[HTML]{B59B81}73 & \cellcolor[HTML]{BA9F7F}72 \\
\itshape Dutch & \itshape Dutch & \cellcolor[HTML]{6C53A4}\color{white} \itbestval{98} & \cellcolor[HTML]{6D54A4}\color{white} \itcell{97} & \cellcolor[HTML]{6F56A3}\color{white} \itcell{97} & \cellcolor[HTML]{7259A1}\color{white} \itcell{95} & \cellcolor[HTML]{79609E}\color{white} \itcell{93} & \cellcolor[HTML]{987E8F}\color{white} \itcell{83} && 
\cellcolor[HTML]{6C53A4}\color{white} \itbestval{97} & \cellcolor[HTML]{6D54A4}\color{white} \itcell{97} & \cellcolor[HTML]{6E55A3}\color{white} \itcell{97} & \cellcolor[HTML]{7057A2}\color{white} \itcell{96} & \cellcolor[HTML]{735AA1}\color{white} \itcell{95} & \cellcolor[HTML]{7B629D}\color{white} \itcell{92} && 
\cellcolor[HTML]{6B52A5}\color{white} \itbestval{98} & \cellcolor[HTML]{6C53A4}\color{white} \itcell{98} & \cellcolor[HTML]{6D54A4}\color{white} \itcell{97} & \cellcolor[HTML]{6F56A3}\color{white} \itcell{96} & \cellcolor[HTML]{7158A2}\color{white} \itcell{96} & \cellcolor[HTML]{785E9F}\color{white} \itcell{94} \\
\\[\spacer]
Bokmål & East N. & \cellcolor[HTML]{F1E6C3}35 & \cellcolor[HTML]{DCC16E}60 & \cellcolor[HTML]{C7AD78}\bestval{67} & \cellcolor[HTML]{CEB375}65 & \cellcolor[HTML]{D5BA72}62 & \cellcolor[HTML]{DDC26E}60 && 
\cellcolor[HTML]{E0C677}57 & \cellcolor[HTML]{DDC26E}\bestval{60} & \cellcolor[HTML]{DFC574}58 & \cellcolor[HTML]{E0C778}57 & \cellcolor[HTML]{E1C87B}56 & \cellcolor[HTML]{E2CB82}54 &&
\cellcolor[HTML]{CAB077}\bestval{66} & \cellcolor[HTML]{D3B972}63 & \cellcolor[HTML]{D3B872}63 & \cellcolor[HTML]{D6BC71}62 & \cellcolor[HTML]{DABF6F}61 & \cellcolor[HTML]{DEC471}59 \\
Bokmål & North N. & \cellcolor[HTML]{F1E5C2}36 & \cellcolor[HTML]{D4B972}63 & \cellcolor[HTML]{C0A67C}\bestval{69} & \cellcolor[HTML]{C7AC78}67 & \cellcolor[HTML]{CEB375}65 &\cellcolor[HTML]{D5BA71}62 &&
\cellcolor[HTML]{DBC06F}61 & \cellcolor[HTML]{D8BD70}\bestval{61} & \cellcolor[HTML]{DAC06F}61 & \cellcolor[HTML]{DDC26E}60 & \cellcolor[HTML]{DEC36F}60 & \cellcolor[HTML]{DFC574}58 && 
\cellcolor[HTML]{BDA37D}\bestval{70} & \cellcolor[HTML]{CAB077}66 & \cellcolor[HTML]{CAB077}66 & \cellcolor[HTML]{CCB276}65 & \cellcolor[HTML]{D0B574}64 & \cellcolor[HTML]{D6BB71}62 \\
Bokmål & West N. & \cellcolor[HTML]{F3E9CB}33 & \cellcolor[HTML]{DEC370}59 & \cellcolor[HTML]{CCB176}\bestval{66} & \cellcolor[HTML]{D3B873}63 & \cellcolor[HTML]{D9BE70}61 & \cellcolor[HTML]{DEC472}59 && 
\cellcolor[HTML]{DFC575}\bestval{58} & \cellcolor[HTML]{DFC677}57 & \cellcolor[HTML]{E1C87C}56 & \cellcolor[HTML]{E2CA80}55 & \cellcolor[HTML]{E2CB82}54 & \cellcolor[HTML]{E3CD87}53 &&
\cellcolor[HTML]{C8AE78}\bestval{67} & \cellcolor[HTML]{D7BD70}62 & \cellcolor[HTML]{D9BE70}61 & \cellcolor[HTML]{DBC06F}60 & \cellcolor[HTML]{DEC370}59 & \cellcolor[HTML]{DFC676}57 \\
Nynorsk & East N. & \cellcolor[HTML]{D0B574}64 & \cellcolor[HTML]{C1A77B}\bestval{69} & \cellcolor[HTML]{C9AE77}67 & \cellcolor[HTML]{CEB375}65 & \cellcolor[HTML]{D7BC71}62 & \cellcolor[HTML]{DEC370}59 &&
\cellcolor[HTML]{DEC370}\bestval{59} & \cellcolor[HTML]{DEC371}59 & \cellcolor[HTML]{E0C87B}56 & \cellcolor[HTML]{E0C77A}56 & \cellcolor[HTML]{E1C97D}55 & \cellcolor[HTML]{E3CD86}53 &&
\cellcolor[HTML]{C8AD78}\bestval{67} & \cellcolor[HTML]{CCB176}66 & \cellcolor[HTML]{D1B674}64 & \cellcolor[HTML]{D5BB71}62 & \cellcolor[HTML]{DBC06E}60 & \cellcolor[HTML]{DFC676}57 \\
Nynorsk & North N. & \cellcolor[HTML]{C6AC79}67 & \cellcolor[HTML]{B89E80}\bestval{72} & \cellcolor[HTML]{C1A67B}69 & \cellcolor[HTML]{C6AB79}68 & \cellcolor[HTML]{CDB275}65 & \cellcolor[HTML]{D4B972}63 &&
\cellcolor[HTML]{D7BC71}\bestval{62} & \cellcolor[HTML]{D9BE70}61 & \cellcolor[HTML]{DEC36F}59 & \cellcolor[HTML]{DCC16E}60 & \cellcolor[HTML]{DEC36F}59 & \cellcolor[HTML]{E0C778}57 &&
\cellcolor[HTML]{BBA07E}\bestval{71} & \cellcolor[HTML]{C4A97A}68 & \cellcolor[HTML]{C8AD78}67 & \cellcolor[HTML]{CCB176}66 & \cellcolor[HTML]{D0B574}64 & \cellcolor[HTML]{D8BD70}62 \\
Nynorsk & West N. & \cellcolor[HTML]{CCB276}65 & \cellcolor[HTML]{C2A87B}\bestval{69} & \cellcolor[HTML]{CCB176}66 & \cellcolor[HTML]{D0B574}64 & \cellcolor[HTML]{D4BA72}63 & \cellcolor[HTML]{DCC16E}60 &&
\cellcolor[HTML]{DFC575}\bestval{58} & \cellcolor[HTML]{DFC576}58 & \cellcolor[HTML]{E0C87B}56 & \cellcolor[HTML]{E0C77A}56 & \cellcolor[HTML]{E1C87C}56 & \cellcolor[HTML]{E3CB84}54 &&
\cellcolor[HTML]{C5AA7A}\bestval{68} & \cellcolor[HTML]{D0B674}64 & \cellcolor[HTML]{D4B972}63 & \cellcolor[HTML]{D8BD70}61 & \cellcolor[HTML]{DBC06F}60 & \cellcolor[HTML]{DFC574}58 \\
\itshape Bokmål & \itshape Bokmål & \cellcolor[HTML]{6950A6}\color{white} \itbestval{99} & \cellcolor[HTML]{6950A6}\color{white} \itcell{98} & \cellcolor[HTML]{6A51A5}\color{white} \itcell{98} & \cellcolor[HTML]{6C53A4}\color{white} \itcell{97} & \cellcolor[HTML]{7057A2}\color{white} \itcell{96} & \cellcolor[HTML]{7F669B}\color{white} \itcell{91} &&
\cellcolor[HTML]{6A51A5}\color{white} \itbestval{98} & \cellcolor[HTML]{6A51A5}\color{white} \itcell{98} & \cellcolor[HTML]{6C53A4}\color{white} \itcell{97} & \cellcolor[HTML]{6E55A3}\color{white} \itcell{97} & \cellcolor[HTML]{7258A2}\color{white} \itcell{96} & \cellcolor[HTML]{7E659C}\color{white} \itcell{92} &&
\cellcolor[HTML]{6950A6}\color{white} \itbestval{99} & \cellcolor[HTML]{6950A6}\color{white} \itcell{98} & \cellcolor[HTML]{6A51A5}\color{white} \itcell{98} & \cellcolor[HTML]{6C53A4}\color{white} \itcell{98} & \cellcolor[HTML]{6F56A3}\color{white} \itcell{97} & \cellcolor[HTML]{795F9E}\color{white} \itcell{93} \\
\itshape Nynorsk & \itshape Nynorsk & \cellcolor[HTML]{6A51A5}\color{white} \itbestval{98} & \cellcolor[HTML]{6B52A5}\color{white} \itcell{98} & \cellcolor[HTML]{6C53A4}\color{white} \itcell{97} & \cellcolor[HTML]{6F56A3}\color{white} \itcell{97} & \cellcolor[HTML]{735AA1}\color{white} \itcell{95} & \cellcolor[HTML]{836999}\color{white} \itcell{90} &&
\cellcolor[HTML]{6C53A4}\color{white} \itbestval{97} & \cellcolor[HTML]{6D54A4}\color{white} \itcell{97} & \cellcolor[HTML]{6F56A3}\color{white} \itcell{96} & \cellcolor[HTML]{7158A2}\color{white} \itcell{96} & \cellcolor[HTML]{765CA0}\color{white} \itcell{94} & \cellcolor[HTML]{81689A}\color{white} \itcell{90} &&
\cellcolor[HTML]{6B52A5}\color{white} \itbestval{98} & \cellcolor[HTML]{6C53A4}\color{white} \itcell{97} & \cellcolor[HTML]{6E55A4}\color{white} \itcell{97} & \cellcolor[HTML]{7056A3}\color{white} \itcell{96} & \cellcolor[HTML]{7359A1}\color{white} \itcell{95} & \cellcolor[HTML]{7B629D}\color{white} \itcell{92} \\
\\[\spacer]
French & Picard & \cellcolor[HTML]{E7D497}48 & \cellcolor[HTML]{E4CE8A}52 & \cellcolor[HTML]{E3CD88}\bestval{52} & \cellcolor[HTML]{E4CE8A}52 & \cellcolor[HTML]{E5CF8D}51 & \cellcolor[HTML]{E7D498}48 &&
\cellcolor[HTML]{C6AB79}68 & \cellcolor[HTML]{B69B81}73 & \cellcolor[HTML]{B49A82}\bestval{74} & \cellcolor[HTML]{B49A82}73 & \cellcolor[HTML]{B69B81}73 & \cellcolor[HTML]{B99F7F}72 &&
\cellcolor[HTML]{C8AE78}67 & \cellcolor[HTML]{B19783}74 & \cellcolor[HTML]{AD9385}\color{white} 76 & \cellcolor[HTML]{AD9385}\color{white} \bestval{76} & \cellcolor[HTML]{AE9484}\color{white} 75 & \cellcolor[HTML]{B09683}\color{white} 75 \\
\itshape French & \itshape French & \cellcolor[HTML]{866D98}\color{white} \itbestval{89} & \cellcolor[HTML]{8A7096}\color{white} \itcell{88} & \cellcolor[HTML]{907693}\color{white} \itcell{86} & \cellcolor[HTML]{987E8F}\color{white} \itcell{83} & \cellcolor[HTML]{A68C88}\color{white} \itcell{78} & \cellcolor[HTML]{CAAF77}\itcell{66} &&
\cellcolor[HTML]{6A51A5}\color{white} \itbestval{98} & \cellcolor[HTML]{6B51A5}\color{white} \itcell{98} & \cellcolor[HTML]{6C53A4}\color{white} \itcell{97} & \cellcolor[HTML]{6C53A4}\color{white} \itcell{97} & \cellcolor[HTML]{7158A2}\color{white} \itcell{96} & \cellcolor[HTML]{7B629D}\color{white} \itcell{93} &&
\cellcolor[HTML]{6950A6}\color{white} \itbestval{98} & \cellcolor[HTML]{6A51A5}\color{white} \itcell{98} & \cellcolor[HTML]{6B52A5}\color{white} \itcell{98} & \cellcolor[HTML]{6C53A5}\color{white} \itcell{98} & \cellcolor[HTML]{6F56A3}\color{white} \itcell{97} & \cellcolor[HTML]{785E9F}\color{white} \itcell{94} \\
\\[\spacer]
French & Occitan* & \cellcolor[HTML]{EDDEB0}41 & \cellcolor[HTML]{EBDAA7}44 & \cellcolor[HTML]{E9D8A1}45 & \cellcolor[HTML]{E9D7A0}\bestval{45} & \cellcolor[HTML]{E9D7A0}45 & \cellcolor[HTML]{EBDAA6}44 && 
\cellcolor[HTML]{8F7594}\color{white} 86 & \cellcolor[HTML]{8C7395}\color{white} \bestval{87} & \cellcolor[HTML]{8F7593}\color{white} 86 & \cellcolor[HTML]{917793}\color{white} 85 & \cellcolor[HTML]{937991}\color{white} 85 & \cellcolor[HTML]{977E8F}\color{white} 83 &&
\cellcolor[HTML]{AA9086}\color{white} 77 & \cellcolor[HTML]{9E848C}\color{white} 81 & \cellcolor[HTML]{987F8F}\color{white} 83 & \cellcolor[HTML]{987E8F}\color{white} \bestval{83} & \cellcolor[HTML]{9A808E}\color{white} 82 & \cellcolor[HTML]{9B818E}\color{white} 82 \\
Spanish & Occitan* & \cellcolor[HTML]{D5BA72}62 & \cellcolor[HTML]{C2A87B}69 & \cellcolor[HTML]{BFA57C}\bestval{70} & \cellcolor[HTML]{C1A67B}69 & \cellcolor[HTML]{C0A67C}69 & \cellcolor[HTML]{C2A77B}69 &&
\cellcolor[HTML]{967C90}\color{white} 83 & \cellcolor[HTML]{947A91}\color{white} \bestval{84} & \cellcolor[HTML]{987E8F}\color{white} 83 & \cellcolor[HTML]{9B818E}\color{white} 82 & \cellcolor[HTML]{9E848C}\color{white} 81 & \cellcolor[HTML]{A48A89}\color{white} 79 &&
\cellcolor[HTML]{B89E80}72 & \cellcolor[HTML]{A58B89}\color{white} \bestval{79} & \cellcolor[HTML]{A68C88}\color{white} 78 & \cellcolor[HTML]{A58B89}\color{white} 79 & \cellcolor[HTML]{A78D88}\color{white} 78 & \cellcolor[HTML]{AA9087}\color{white} 77 \\
\itshape Spanish & \itshape Spanish & \cellcolor[HTML]{674EA7}\color{white} \itbestval{99} & \cellcolor[HTML]{684FA6}\color{white} \itshape 99 & \cellcolor[HTML]{6C53A4}\color{white} \itcell{97} & \cellcolor[HTML]{6D54A4}\color{white} \itcell{97} & \cellcolor[HTML]{7158A2}\color{white} \itcell{96} & \cellcolor[HTML]{866D98}\color{white} \itcell{89} &&
\cellcolor[HTML]{684FA6}\color{white} \itbestval{99} & \cellcolor[HTML]{684FA6}\color{white} \itshape 99 & \cellcolor[HTML]{6B52A5}\color{white} \itcell{98} & \cellcolor[HTML]{6F56A3}\color{white} \itcell{96} & \cellcolor[HTML]{7057A2}\color{white} \itcell{96} & \cellcolor[HTML]{7E659B}\color{white} \itcell{91} &&
\cellcolor[HTML]{684FA6}\color{white} \itbestval{99} & \cellcolor[HTML]{684FA6}\color{white} \itshape 99 & \cellcolor[HTML]{6950A6}\color{white} \itcell{98} & \cellcolor[HTML]{6B52A5}\color{white} \itcell{98} & \cellcolor[HTML]{6D54A4}\color{white} \itcell{97} & \cellcolor[HTML]{785F9E}\color{white} \itcell{93} \\
\\[\spacer]
MSA & Egyptian A. & \cellcolor[HTML]{C7AC78}67 & \cellcolor[HTML]{BFA57C}\bestval{70} & \cellcolor[HTML]{C9AE77}66 & \cellcolor[HTML]{D6BB71}62 & \cellcolor[HTML]{E0C779}57 & \cellcolor[HTML]{E5D08E}50 &&
\cellcolor[HTML]{DEC472}59 & \cellcolor[HTML]{D9BE6F}\bestval{61} & \cellcolor[HTML]{DDC26E}60 & \cellcolor[HTML]{DFC575}58 & \cellcolor[HTML]{E2CB84}54 & \cellcolor[HTML]{E7D499}47 &&
\cellcolor[HTML]{D2B773}64 & \cellcolor[HTML]{C9AE77}\bestval{66} & \cellcolor[HTML]{CCB176}65 & \cellcolor[HTML]{D7BC71}62 & \cellcolor[HTML]{DFC677}57 & \cellcolor[HTML]{E6D191}50 \\
MSA & Gulf Arabic & \cellcolor[HTML]{C9AF77}66 & \cellcolor[HTML]{C1A77B}\bestval{69} & \cellcolor[HTML]{CCB276}65 & \cellcolor[HTML]{D8BE70}61 & \cellcolor[HTML]{E1C87C}56 & \cellcolor[HTML]{E6D292}49 &&
\cellcolor[HTML]{CCB276}\bestval{65} & \cellcolor[HTML]{CDB375}65 & \cellcolor[HTML]{D6BB71}62 & \cellcolor[HTML]{DEC36F}60 & \cellcolor[HTML]{E1C97E}55 & \cellcolor[HTML]{E6D293}49 &&
\cellcolor[HTML]{CBB076}66 & \cellcolor[HTML]{CAAF77}\bestval{66} & \cellcolor[HTML]{CEB475}65 & \cellcolor[HTML]{D9BE70}61 & \cellcolor[HTML]{E0C779}57 & \cellcolor[HTML]{E6D192}49 \\
MSA & Levantine A. & \cellcolor[HTML]{D1B674}64 & \cellcolor[HTML]{CDB375}\bestval{65} & \cellcolor[HTML]{D6BB71}62 & \cellcolor[HTML]{DFC473}58 & \cellcolor[HTML]{E3CC86}53 & \cellcolor[HTML]{E8D59B}47 &&
\cellcolor[HTML]{E1C87C}56 & \cellcolor[HTML]{E0C778}\bestval{57} & \cellcolor[HTML]{E1C97F}55 & \cellcolor[HTML]{E3CC84}53 & \cellcolor[HTML]{E6D191}50 & \cellcolor[HTML]{EAD9A3}45 &&
\cellcolor[HTML]{DEC471}59 & \cellcolor[HTML]{DABF6F}\bestval{61} & \cellcolor[HTML]{DDC26E}60 & \cellcolor[HTML]{E0C778}57 & \cellcolor[HTML]{E3CC86}53 & \cellcolor[HTML]{E8D69D}46 \\
MSA & Maghrebi A. & \cellcolor[HTML]{E5D08E}51 & \cellcolor[HTML]{E2CA81}\bestval{54} & \cellcolor[HTML]{E3CC86}53 & \cellcolor[HTML]{E5D08F}50 & \cellcolor[HTML]{E8D69D}46 & \cellcolor[HTML]{ECDCAC}42 &&
\cellcolor[HTML]{E5D090}50 & \cellcolor[HTML]{E5D08E}\bestval{51} & \cellcolor[HTML]{E6D292}49 & \cellcolor[HTML]{E7D396}48 & \cellcolor[HTML]{E9D79E}46 & \cellcolor[HTML]{ECDCAB}42 &&
\cellcolor[HTML]{E5CF8D}51 & \cellcolor[HTML]{E3CC86}\bestval{53} & \cellcolor[HTML]{E3CD88}52 & \cellcolor[HTML]{E5D08F}50 & \cellcolor[HTML]{E8D59B}47 & \cellcolor[HTML]{EBDCAA}42 \\
\itshape MSA & \itshape MSA & \cellcolor[HTML]{765D9F}\color{white} \itbestval{94} & \cellcolor[HTML]{7A619E}\color{white} \itcell{93} & \cellcolor[HTML]{866C98}\color{white} \itcell{89} & \cellcolor[HTML]{987F8F}\color{white} \itcell{83} & \cellcolor[HTML]{A68C88}\color{white} \itcell{78} & \cellcolor[HTML]{C8AD78}\itcell{67} &&
\cellcolor[HTML]{7057A2}\color{white} \itbestval{96} & \cellcolor[HTML]{745AA1}\color{white} \itcell{95} & \cellcolor[HTML]{7F659B}\color{white} \itcell{91} & \cellcolor[HTML]{907693}\color{white} \itcell{85} & \cellcolor[HTML]{A3898A}\color{white} \itcell{79} & \cellcolor[HTML]{C2A77B}\itcell{69} &&
\cellcolor[HTML]{6F56A3}\color{white} \itbestval{96} & \cellcolor[HTML]{735AA1}\color{white} \itcell{95} & \cellcolor[HTML]{7E659C}\color{white} \itcell{91} & \cellcolor[HTML]{8E7494}\color{white} \itcell{86} & \cellcolor[HTML]{A1878B}\color{white} \itcell{80} & \cellcolor[HTML]{BDA37D}\itcell{70} \\
\\[\spacer]
Finnish & Ostroboth. F. & \cellcolor[HTML]{9D838D}\color{white} \bestval{81} & \cellcolor[HTML]{A0868B}\color{white} 80 & \cellcolor[HTML]{A58B89}\color{white} 79 & \cellcolor[HTML]{A88E87}\color{white} 77 & \cellcolor[HTML]{A78D88}\color{white} 78 & \cellcolor[HTML]{AF9584}\color{white} 75 &&
\cellcolor[HTML]{A78D88}\color{white} 78 & \cellcolor[HTML]{A58B89}\color{white} \bestval{78} & \cellcolor[HTML]{AB9186}\color{white} 76 & \cellcolor[HTML]{B49982}74 & \cellcolor[HTML]{B59B81}73 & \cellcolor[HTML]{BEA47D}70 &&
\cellcolor[HTML]{9D838D}\color{white} 81 & \cellcolor[HTML]{917793}\color{white} 85 & \cellcolor[HTML]{8E7494}\color{white} 86 & \cellcolor[HTML]{8E7494}\color{white} \bestval{86} & \cellcolor[HTML]{8F7594}\color{white} 86 & \cellcolor[HTML]{937A91}\color{white} 84 \\
Finnish & SE Finnish & \cellcolor[HTML]{9D838D}\color{white} \bestval{81} & \cellcolor[HTML]{A48A89}\color{white} 79 & \cellcolor[HTML]{AA9086}\color{white} 77 & \cellcolor[HTML]{AF9484}\color{white} 75 & \cellcolor[HTML]{AD9385}\color{white} 76 & \cellcolor[HTML]{B69B81}\color{white} 73 &&
\cellcolor[HTML]{B09683}\color{white} 75 & \cellcolor[HTML]{AF9484}\color{white} \bestval{75} & \cellcolor[HTML]{B69C81}\color{white} 73 & \cellcolor[HTML]{BFA47C}70 & \cellcolor[HTML]{C1A77B}69 & \cellcolor[HTML]{CAAF77}66 &&
\cellcolor[HTML]{9F858C}\color{white} 81 & \cellcolor[HTML]{957B90}\color{white} 84 & \cellcolor[HTML]{947A91}\color{white} 84 & \cellcolor[HTML]{947A91}\color{white} \bestval{84} & \cellcolor[HTML]{957B91}\color{white} 84 & \cellcolor[HTML]{9A808E}\color{white} 82 \\
Finnish & SW Finnish & \cellcolor[HTML]{B09683}\color{white} \bestval{75} & \cellcolor[HTML]{B59B81}\color{white} 73 & \cellcolor[HTML]{B99F7F}\color{white} 72 & \cellcolor[HTML]{BCA27D}\color{white} 71 & \cellcolor[HTML]{BAA07F}\color{white} 71 & \cellcolor[HTML]{C0A57C}70 &&
\cellcolor[HTML]{C4A97A} \bestval{68} & \cellcolor[HTML]{C4AA7A} 68 & \cellcolor[HTML]{C8AE78}67 & \cellcolor[HTML]{D1B674}64 & \cellcolor[HTML]{D2B873}63 & \cellcolor[HTML]{DABF6F}61 &&
\cellcolor[HTML]{AD9385}\color{white} 76 & \cellcolor[HTML]{A2888A}\color{white} 80 & \cellcolor[HTML]{9F858B}\color{white} 80 & \cellcolor[HTML]{9F858C}\color{white} \bestval{81} & \cellcolor[HTML]{9F858C}\color{white} 81 & \cellcolor[HTML]{A58B89}\color{white} 79 \\
Finnish & SW trans. area & \cellcolor[HTML]{A58B89}\color{white} \bestval{79} & \cellcolor[HTML]{A78D88}\color{white} 78 & \cellcolor[HTML]{AA9086}\color{white} 77 & \cellcolor[HTML]{AD9385}\color{white} 76 & \cellcolor[HTML]{AB9186}\color{white} 76 & \cellcolor[HTML]{B29783}74 &&
\cellcolor[HTML]{B99F7F}\bestval{72} & \cellcolor[HTML]{BA9F7F}72 & \cellcolor[HTML]{BDA37D}70 & \cellcolor[HTML]{C4AA7A}68 & \cellcolor[HTML]{C6AB79}67 & \cellcolor[HTML]{CDB375}65 &&
\cellcolor[HTML]{A4898A}\color{white} 79 & \cellcolor[HTML]{957B90}\color{white} 84 & \cellcolor[HTML]{937991}\color{white} 84 & \cellcolor[HTML]{937992}\color{white} \bestval{85} & \cellcolor[HTML]{937A91}\color{white} 84 & \cellcolor[HTML]{997F8F}\color{white} 83 \\
Finnish & Savonian F. & \cellcolor[HTML]{9A808E}\color{white} \bestval{82} & \cellcolor[HTML]{A0868B}\color{white} 80 & \cellcolor[HTML]{A78D88}\color{white} 78 & \cellcolor[HTML]{AD9285}\color{white} 76 & \cellcolor[HTML]{AB9186}\color{white} 76 & \cellcolor[HTML]{B49A81}73 &&
\cellcolor[HTML]{A88E87}\color{white} 77 & \cellcolor[HTML]{A58B89}\color{white} \bestval{79} & \cellcolor[HTML]{AC9285}\color{white} 76 & \cellcolor[HTML]{B59B81}73 & \cellcolor[HTML]{B89D80}72 & \cellcolor[HTML]{C1A77B}69 &&
\cellcolor[HTML]{9C828D}\color{white} 81 & \cellcolor[HTML]{937A91}\color{white} 84 & \cellcolor[HTML]{927892}\color{white} 85 & \cellcolor[HTML]{917793}\color{white} \bestval{85} & \cellcolor[HTML]{927892}\color{white} 85 & \cellcolor[HTML]{987E8F}\color{white} 83 \\
Finnish & Tavastian F. & \cellcolor[HTML]{9C828D}\color{white} \bestval{81} & \cellcolor[HTML]{9F858C}\color{white} 80 & \cellcolor[HTML]{A48A89}\color{white} 79 & \cellcolor[HTML]{A88E87}\color{white} 78 & \cellcolor[HTML]{A78D88}\color{white} 78 & \cellcolor[HTML]{AE9484}\color{white} 75 &&
\cellcolor[HTML]{AC9285}\color{white} 76 & \cellcolor[HTML]{AA8F87}\color{white} \bestval{77} & \cellcolor[HTML]{AE9485}\color{white} 76 & \cellcolor[HTML]{B69B81}73 & \cellcolor[HTML]{B89D80}72 & \cellcolor[HTML]{C1A67B}69 &&
\cellcolor[HTML]{9E848C}\color{white} 81 & \cellcolor[HTML]{927892}\color{white} 85 & \cellcolor[HTML]{8F7594}\color{white} 86 & \cellcolor[HTML]{8E7594}\color{white} \bestval{86} & \cellcolor[HTML]{8F7593}\color{white} 86 & \cellcolor[HTML]{937A91}\color{white} 84 \\
\itshape Finnish & \itshape Finnish & \cellcolor[HTML]{6A51A5}\color{white} \itbestval{98} & \cellcolor[HTML]{6A51A5}\color{white} \itcell{98} & \cellcolor[HTML]{6B52A5}\color{white} \itcell{98} & \cellcolor[HTML]{6D54A4}\color{white} \itcell{97} & \cellcolor[HTML]{7057A2}\color{white} \itcell{96} & \cellcolor[HTML]{785E9F}\color{white} \itcell{94} &&
\cellcolor[HTML]{6F56A3}\color{white} \itbestval{96} & \cellcolor[HTML]{7057A2}\color{white} \itcell{96} & \cellcolor[HTML]{7158A2}\color{white} \itcell{96} & \cellcolor[HTML]{735AA1}\color{white} \itcell{95} & \cellcolor[HTML]{755CA0}\color{white} \itcell{94} & \cellcolor[HTML]{7A619E}\color{white} \itcell{93} &&
\cellcolor[HTML]{6B52A5}\color{white} \itbestval{98} & \cellcolor[HTML]{6C53A4}\color{white} \itcell{97} & \cellcolor[HTML]{6D54A4}\color{white} \itcell{97} & \cellcolor[HTML]{6E55A3}\color{white} \itcell{97} & \cellcolor[HTML]{7056A3}\color{white} \itcell{96} & \cellcolor[HTML]{765D9F}\color{white} \itcell{94}\\
\bottomrule
\end{tabular}

==> tables/corr-seen-subwords.tex <==
\begin{tabular}{@{}l@{\hspace{2mm}}l
S[table-format=+1.2]S[table-format=1.2]
S[table-format=+1.2]S[table-format=1.2]
S[table-format=+1.2]S[table-format=1.2]@{}
}
\toprule
\textbf{Src} & \textbf{Target} & \multicolumn{2}{c}{\textbf{Monoling.}} & \multicolumn{2}{c}{\textbf{mBERT}} & \multicolumn{2}{c}{\textbf{XLM-R}} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}
 &  & \multicolumn{1}{c}{$\rho$} & \multicolumn{1}{c}{p} & \multicolumn{1}{c}{$\rho$} & \multicolumn{1}{c}{p} & \multicolumn{1}{c}{$\rho$} & \multicolumn{1}{c}{p} \\
 \midrule
Ger. & Als. G. & \cellcolor[HTML]{FFF7DD}0.34 & 0.03 & \cellcolor[HTML]{FFEFC0}0.62 & 0.00 & \cellcolor[HTML]{FFEEB9}0.69 & 0.00 \\
Ger. & Swiss G. & \cellcolor[HTML]{FFEBB0}0.78 & 0.00 & \cellcolor[HTML]{FFEBAF}0.79 & 0.00 & \cellcolor[HTML]{FFEFBF}0.64 & 0.00 \\
Ger. & L. Saxon & \cellcolor[HTML]{FFF5D7}0.40 & 0.01 & \cellcolor[HTML]{FFEDB5}0.73 & 0.00 & \cellcolor[HTML]{FFE9A7}0.86 & 0.00 \\
Dutch & L. Saxon & \cellcolor[HTML]{FFECB3}0.75 & 0.00 & \cellcolor[HTML]{CEE0F0}-0.25 & \cellcolor[HTML]{CCCCCC}0.19 & \cellcolor[HTML]{FFEEBB}0.68 & 0.00 \\
Bokm. & East N. & \cellcolor[HTML]{FFF8E1}0.30 & \cellcolor[HTML]{CCCCCC}0.11 & \cellcolor[HTML]{82B0DA}-0.64 & 0.00 & \cellcolor[HTML]{669ED2}-0.79 & 0.00 \\
Bokm. & North N. & \cellcolor[HTML]{FFF8E1}0.29 & \cellcolor[HTML]{CCCCCC}0.11 & \cellcolor[HTML]{9CC0E1}-0.51 & 0.01 & \cellcolor[HTML]{72A6D5}-0.72 & 0.00 \\
Bokm. & West N. & \cellcolor[HTML]{FFFAE9}0.22 & \cellcolor[HTML]{CCCCCC}0.25 & \cellcolor[HTML]{6BA2D3}-0.76 & 0.00 & \cellcolor[HTML]{629CD1}-0.80 & 0.00 \\
Nynor. & East N. & \cellcolor[HTML]{BAD3EA}-0.36 & \cellcolor[HTML]{CCCCCC}0.05 & \cellcolor[HTML]{81B0DA}-0.64 & 0.00 & \cellcolor[HTML]{5F9AD0}-0.82 & 0.00 \\
Nynor. & North N. & \cellcolor[HTML]{ADCBE7}-0.42 & 0.02 & \cellcolor[HTML]{93BBDF}-0.56 & 0.00 & \cellcolor[HTML]{639DD1}-0.80 & 0.00 \\
Nynor. & West N. & \cellcolor[HTML]{86B3DB}-0.62 & 0.00 & \cellcolor[HTML]{74A7D6}-0.71 & 0.00 & \cellcolor[HTML]{629CD0}-0.81 & 0.00 \\
French & Picard & \cellcolor[HTML]{FFEAAC}0.82 & 0.00 & \cellcolor[HTML]{FFF9E7}0.24 & \cellcolor[HTML]{CCCCCC}0.21 & \cellcolor[HTML]{FFF2CB}0.52 & 0.00 \\
French & Occitan & \cellcolor[HTML]{FFEEBC}0.66 & 0.00 & \cellcolor[HTML]{659ED1}-0.79 & 0.00 & \cellcolor[HTML]{FFF3CF}0.48 & 0.01 \\
Spa. & Occitan & \cellcolor[HTML]{FFEEB9}0.69 & 0.00 & \cellcolor[HTML]{5594CD}-0.87 & 0.00 & \cellcolor[HTML]{FFFCF0}0.15 & \cellcolor[HTML]{CCCCCC}0.44 \\
MSA & Egy. A. & \cellcolor[HTML]{B8D2EA}-0.36 & 0.05 & \cellcolor[HTML]{FFF8E4}0.27 & \cellcolor[HTML]{CCCCCC}0.14 & \cellcolor[HTML]{FFF1C5}0.57 & 0.00 \\
MSA & Gulf A. & \cellcolor[HTML]{91BADE}-0.56 & 0.00 & \cellcolor[HTML]{AECCE7}-0.41 & 0.02 & \cellcolor[HTML]{FBFDFE}-0.02 & \cellcolor[HTML]{CCCCCC}0.94 \\
MSA & Lev. A. & \cellcolor[HTML]{8DB7DD}-0.58 & 0.00 & \cellcolor[HTML]{C5DAEE}-0.30 & \cellcolor[HTML]{CCCCCC}0.11 & \cellcolor[HTML]{FFF7DE}0.33 & \cellcolor[HTML]{CCCCCC}0.11 \\
MSA & Mag. A. & \cellcolor[HTML]{D2E2F1}-0.23 & \cellcolor[HTML]{CCCCCC}0.22 & \cellcolor[HTML]{CDDFF0}-0.26 & \cellcolor[HTML]{CCCCCC}0.17 & \cellcolor[HTML]{FFF9E4}0.27 & \cellcolor[HTML]{CCCCCC}0.20 \\
Fin. & Ost. F. & \cellcolor[HTML]{FFFFFF}0.01 & \cellcolor[HTML]{CCCCCC}0.98 & \cellcolor[HTML]{659ED1}-0.79 & 0.00 & \cellcolor[HTML]{FFF4D3}0.44 & 0.01 \\
Fin. & SE F. & \cellcolor[HTML]{F1F6FA}-0.07 & \cellcolor[HTML]{CCCCCC}0.71 & \cellcolor[HTML]{70A5D5}-0.73 & 0.00 & \cellcolor[HTML]{FFF5D6}0.40 & 0.03 \\
Fin. & SW F. & \cellcolor[HTML]{B8D2EA}-0.37 & 0.05 & \cellcolor[HTML]{5C98CF}-0.84 & 0.00 & \cellcolor[HTML]{FFF7DC}0.35 & \cellcolor[HTML]{CCCCCC}0.06 \\
Fin. & SW tr. & \cellcolor[HTML]{E7F0F8}-0.12 & \cellcolor[HTML]{CCCCCC}0.52 & \cellcolor[HTML]{5E99CF}-0.83 & 0.00 & \cellcolor[HTML]{FFF6DA}0.37 & 0.05 \\
Fin. & Sav. F. & \cellcolor[HTML]{FFFFFE}0.01 & \cellcolor[HTML]{CCCCCC}0.95 & \cellcolor[HTML]{68A0D2}-0.77 & 0.00 & \cellcolor[HTML]{FFF3D0}0.47 & 0.01 \\
Fin. & Tav. F. & \cellcolor[HTML]{F3F7FB}-0.06 & \cellcolor[HTML]{CCCCCC}0.75 & \cellcolor[HTML]{71A6D5}-0.73 & 0.00 & \cellcolor[HTML]{FFF1C6}0.57 & 0.00 \\ \bottomrule
\end{tabular}

==> tables/corr-seen-words.tex <==
\begin{tabular}{@{}l@{\hspace{2mm}}l
S[table-format=+1.2]S[table-format=1.2]
S[table-format=+1.2]S[table-format=1.2]
S[table-format=+1.2]S[table-format=1.2]@{}
}
\toprule
\textbf{Src} & \textbf{Target} & \multicolumn{2}{c}{\textbf{Monoling.}} & \multicolumn{2}{c}{\textbf{mBERT}} & \multicolumn{2}{c}{\textbf{XLM-R}} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}
 &  & \multicolumn{1}{c}{$\rho$} & \multicolumn{1}{c}{p} & \multicolumn{1}{c}{$\rho$} & \multicolumn{1}{c}{p} & \multicolumn{1}{c}{$\rho$} & \multicolumn{1}{c}{p} \\
 \midrule
Ger. & Als. G. & \cellcolor[HTML]{FFE8A5}0.89 & 0.00 & \cellcolor[HTML]{FFECB1}0.77 & 0.00 & \cellcolor[HTML]{FFE9A9}0.85 & 0.00 \\
Ger. & Swiss G. & \cellcolor[HTML]{FFEAAD}0.81 & 0.00 & \cellcolor[HTML]{FFECB2}0.76 & 0.00 & \cellcolor[HTML]{FFEAAA}0.84 & 0.00 \\
Ger. & L. Saxon & \cellcolor[HTML]{FFE9A8}0.86 & 0.00 & \cellcolor[HTML]{FFEDB6}0.72 & 0.00 & \cellcolor[HTML]{FFE9A6}0.88 & 0.00 \\
Dutch & L. Saxon & \cellcolor[HTML]{FFECB4}0.74 & 0.00 & \cellcolor[HTML]{FFF9E5}0.26 & \cellcolor[HTML]{CCCCCC}0.16 & \cellcolor[HTML]{FFEBAF}0.79 & 0.00 \\
Bokm. & East N. & \cellcolor[HTML]{FFF8E1}0.30 & \cellcolor[HTML]{CCCCCC}0.11 & \cellcolor[HTML]{7FAED9}-0.66 & 0.00 & \cellcolor[HTML]{76A9D7}-0.70 & 0.00 \\
Bokm. & North N. & \cellcolor[HTML]{FFF6DA}0.37 & 0.04 & \cellcolor[HTML]{80AFD9}-0.65 & 0.00 & \cellcolor[HTML]{8DB7DD}-0.59 & 0.00 \\
Bokm. & West N. & \cellcolor[HTML]{FFF9E8}0.23 & \cellcolor[HTML]{CCCCCC}0.21 & \cellcolor[HTML]{619BD0}-0.81 & 0.00 & \cellcolor[HTML]{7BACD8}-0.68 & 0.00 \\
Nynor. & East N. & \cellcolor[HTML]{A2C5E3}-0.48 & 0.01 & \cellcolor[HTML]{6CA2D3}-0.76 & 0.00 & \cellcolor[HTML]{5896CD}-0.86 & 0.00 \\
Nynor. & North N. & \cellcolor[HTML]{99BFE1}-0.52 & 0.00 & \cellcolor[HTML]{88B4DC}-0.61 & 0.00 & \cellcolor[HTML]{69A0D2}-0.77 & 0.00 \\
Nynor. & West N. & \cellcolor[HTML]{8CB6DD}-0.59 & 0.00 & \cellcolor[HTML]{87B3DB}-0.62 & 0.00 & \cellcolor[HTML]{659ED1}-0.79 & 0.00 \\
French & Picard & \cellcolor[HTML]{FFF2CC}0.51 & 0.00 & \cellcolor[HTML]{FFEFC0}0.62 & 0.00 & \cellcolor[HTML]{FFEBAF}0.79 & 0.00 \\
French & Occitan & \cellcolor[HTML]{FFEAAC}0.82 & 0.00 & \cellcolor[HTML]{9DC1E2}-0.50 & 0.00 & \cellcolor[HTML]{FFEBB1}0.77 & 0.00 \\
Spa. & Occitan & \cellcolor[HTML]{FFF2CC}0.51 & 0.00 & \cellcolor[HTML]{98BEE0}-0.53 & 0.00 & \cellcolor[HTML]{FFF4D3}0.44 & 0.01 \\
MSA & Egy. A. & \cellcolor[HTML]{FFFBEE}0.17 & \cellcolor[HTML]{CCCCCC}0.38 & \cellcolor[HTML]{FFF5D8}0.39 & 0.03 & \cellcolor[HTML]{FFF8E2}0.29 & \cellcolor[HTML]{CCCCCC}0.12 \\
MSA & Gulf A. & \cellcolor[HTML]{FFFFFE}0.01 & \cellcolor[HTML]{CCCCCC}0.96 & \cellcolor[HTML]{FFFFFC}0.04 & \cellcolor[HTML]{CCCCCC}0.85 & \cellcolor[HTML]{C9DDEF}-0.27 & \cellcolor[HTML]{CCCCCC}0.19 \\
MSA & Lev. A. & \cellcolor[HTML]{FFFEF8}0.07 & \cellcolor[HTML]{CCCCCC}0.72 & \cellcolor[HTML]{FFFCF4}0.12 & \cellcolor[HTML]{CCCCCC}0.54 & \cellcolor[HTML]{EEF4FA}-0.08 & \cellcolor[HTML]{CCCCCC}0.69 \\
MSA & Mag. A. & \cellcolor[HTML]{FFF8E1}0.30 & \cellcolor[HTML]{CCCCCC}0.11 & \cellcolor[HTML]{FFFFFE}0.02 & \cellcolor[HTML]{CCCCCC}0.93 & \cellcolor[HTML]{F9FBFD}-0.03 & \cellcolor[HTML]{CCCCCC}0.90 \\
Fin. & Ost. F. & \cellcolor[HTML]{FFF9E8}0.23 & \cellcolor[HTML]{CCCCCC}0.22 & \cellcolor[HTML]{FFF5D6}0.41 & 0.02 & \cellcolor[HTML]{FFF0C1}0.62 & 0.00 \\
Fin. & SE F. & \cellcolor[HTML]{E9F1F8}-0.11 & \cellcolor[HTML]{CCCCCC}0.55 & \cellcolor[HTML]{FFFFFE}0.01 & \cellcolor[HTML]{CCCCCC}0.94 & \cellcolor[HTML]{FFECB2}0.76 & 0.00 \\
Fin. & SW F. & \cellcolor[HTML]{BCD5EB}-0.34 & \cellcolor[HTML]{CCCCCC}0.06 & \cellcolor[HTML]{E1ECF6}-0.15 & \cellcolor[HTML]{CCCCCC}0.42 & \cellcolor[HTML]{FFEEB9}0.69 & 0.00 \\
Fin. & SW tr. & \cellcolor[HTML]{FFF6DB}0.36 & \cellcolor[HTML]{CCCCCC}0.05 & \cellcolor[HTML]{FFF3CD}0.49 & 0.01 & \cellcolor[HTML]{FFF4D2}0.44 & 0.01 \\
Fin. & Sav. F. & \cellcolor[HTML]{FFFBF0}0.16 & \cellcolor[HTML]{CCCCCC}0.41 & \cellcolor[HTML]{FFF8E3}0.28 & \cellcolor[HTML]{CCCCCC}0.13 & \cellcolor[HTML]{FFECB3}0.75 & 0.00 \\
Fin. & Tav. F. & \cellcolor[HTML]{FFF9E7}0.24 & \cellcolor[HTML]{CCCCCC}0.20 & \cellcolor[HTML]{FFF3CD}0.50 & 0.01 & \cellcolor[HTML]{FFF0C1}0.61 & 0.00 \\ \bottomrule
\end{tabular}

==> tables/corr-ttr-ratio.tex <==
\begin{tabular}{@{}l@{\hspace{2mm}}l
S[table-format=+1.2]S[table-format=1.2]
S[table-format=+1.2]S[table-format=1.2]
S[table-format=+1.2]S[table-format=1.2]@{}
}
\toprule
\textbf{Src} & \textbf{Target} & \multicolumn{2}{c}{\textbf{Monoling.}} & \multicolumn{2}{c}{\textbf{mBERT}} & \multicolumn{2}{c}{\textbf{XLM-R}} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}
 &  & \multicolumn{1}{c}{$\rho$} & \multicolumn{1}{c}{p} & \multicolumn{1}{c}{$\rho$} & \multicolumn{1}{c}{p} & \multicolumn{1}{c}{$\rho$} & \multicolumn{1}{c}{p} \\
 \midrule
 Ger. & Als. G. & \cellcolor[HTML]{FFE9A7}0.87 & 0.00 & \cellcolor[HTML]{FFF6DA}0.37 & 0.05 & \cellcolor[HTML]{FFF2C9}0.53 & 0.00 \\
Ger. & Swiss G. & \cellcolor[HTML]{FFEEBB}0.67 & 0.00 & \cellcolor[HTML]{FFFDF4}0.11 & \cellcolor[HTML]{CCCCCC}0.57 & \cellcolor[HTML]{FFFAEA}0.21 & \cellcolor[HTML]{CCCCCC}0.26 \\
Ger. & L. Saxon & \cellcolor[HTML]{FFE8A4}0.90 & 0.00 & \cellcolor[HTML]{FFEFC1}0.62 & 0.00 & \cellcolor[HTML]{FFEDB9}0.69 & 0.00 \\
Dutch & L. Saxon & \cellcolor[HTML]{FFF2C9}0.53 & 0.00 & \cellcolor[HTML]{9DC1E2}-0.50 & 0.00 & \cellcolor[HTML]{FFFCF1}0.15 & \cellcolor[HTML]{CCCCCC}0.44 \\
Bokm. & East N. & \cellcolor[HTML]{FFFBF0}0.16 & \cellcolor[HTML]{CCCCCC}0.41 & \cellcolor[HTML]{649DD1}-0.80 & 0.00 & \cellcolor[HTML]{9FC3E2}-0.49 & 0.01 \\
Bokm. & North N. & \cellcolor[HTML]{FFFCF0}0.15 & \cellcolor[HTML]{CCCCCC}0.44 & \cellcolor[HTML]{7CADD8}-0.67 & 0.00 & \cellcolor[HTML]{A7C7E5}-0.45 & 0.01 \\
Bokm. & West N. & \cellcolor[HTML]{FFFCF2}0.13 & \cellcolor[HTML]{CCCCCC}0.49 & \cellcolor[HTML]{70A5D5}-0.73 & 0.00 & \cellcolor[HTML]{92BADF}-0.56 & 0.00 \\
Nynor. & East N. & \cellcolor[HTML]{5D99CF}-0.83 & 0.00 & \cellcolor[HTML]{81B0DA}-0.65 & 0.00 & \cellcolor[HTML]{ECF3F9}-0.10 & \cellcolor[HTML]{CCCCCC}0.62 \\
Nynor. & North N. & \cellcolor[HTML]{5997CE}-0.85 & 0.00 & \cellcolor[HTML]{A4C6E4}-0.47 & 0.01 & \cellcolor[HTML]{F5F9FC}-0.05 & \cellcolor[HTML]{CCCCCC}0.80 \\
Nynor. & West N. & \cellcolor[HTML]{4D8FCA}-0.92 & 0.00 & \cellcolor[HTML]{89B5DC}-0.61 & 0.00 & \cellcolor[HTML]{F2F7FB}-0.06 & \cellcolor[HTML]{CCCCCC}0.74 \\
French & Picard & \cellcolor[HTML]{E3EDF6}-0.14 & \cellcolor[HTML]{CCCCCC}0.45 & \cellcolor[HTML]{FFFBF0}0.15 & \cellcolor[HTML]{CCCCCC}0.42 & \cellcolor[HTML]{FFF7DE}0.33 & \cellcolor[HTML]{CCCCCC}0.07 \\
French & Occitan & \cellcolor[HTML]{FFF4D2}0.45 & 0.01 & \cellcolor[HTML]{5D99CF}-0.83 & 0.00 & \cellcolor[HTML]{FFF5D8}0.39 & 0.03 \\
Spa. & Occitan & \cellcolor[HTML]{FFF6DB}0.36 & \cellcolor[HTML]{CCCCCC}0.05 & \cellcolor[HTML]{458AC8}-0.95 & 0.00 & \cellcolor[HTML]{B0CDE7}-0.41 & 0.03 \\
MSA & Egy. A. & \cellcolor[HTML]{B5D0E9}-0.38 & 0.04 & \cellcolor[HTML]{68A0D2}-0.77 & 0.00 & \cellcolor[HTML]{609BD0}-0.82 & 0.00 \\
MSA & Gulf A. & \cellcolor[HTML]{B8D2EA}-0.37 & 0.05 & \cellcolor[HTML]{468BC8}-0.95 & 0.00 & \cellcolor[HTML]{5191CC}-0.89 & 0.00 \\
MSA & Lev. A. & \cellcolor[HTML]{C3D9ED}-0.31 & \cellcolor[HTML]{CCCCCC}0.10 & \cellcolor[HTML]{4E90CB}-0.91 & 0.00 & \cellcolor[HTML]{5B98CE}-0.84 & 0.00 \\
MSA & Mag. A. & \cellcolor[HTML]{84B1DA}-0.63 & 0.00 & \cellcolor[HTML]{5694CD}-0.87 & 0.00 & \cellcolor[HTML]{71A5D5}-0.73 & 0.00 \\
Fin. & Ost. F. & \cellcolor[HTML]{5694CD}-0.87 & 0.00 & \cellcolor[HTML]{6CA3D4}-0.75 & 0.00 & \cellcolor[HTML]{F8FBFD}-0.03 & \cellcolor[HTML]{CCCCCC}0.87 \\
Fin. & SE F. & \cellcolor[HTML]{5594CD}-0.87 & 0.00 & \cellcolor[HTML]{6AA1D3}-0.76 & 0.00 & \cellcolor[HTML]{DEEAF5}-0.17 & \cellcolor[HTML]{CCCCCC}0.38 \\
Fin. & SW F. & \cellcolor[HTML]{629CD1}-0.81 & 0.00 & \cellcolor[HTML]{75A8D6}-0.71 & 0.00 & \cellcolor[HTML]{F0F5FA}-0.08 & \cellcolor[HTML]{CCCCCC}0.69 \\
Fin. & SW tr. & \cellcolor[HTML]{619BD0}-0.81 & 0.00 & \cellcolor[HTML]{78AAD7}-0.69 & 0.00 & \cellcolor[HTML]{EBF2F9}-0.10 & \cellcolor[HTML]{CCCCCC}0.60 \\
Fin. & Sav. F. & \cellcolor[HTML]{5694CD}-0.87 & 0.00 & \cellcolor[HTML]{69A1D3}-0.77 & 0.00 & \cellcolor[HTML]{EDF3F9}-0.09 & \cellcolor[HTML]{CCCCCC}0.63 \\
Fin. & Tav. F. & \cellcolor[HTML]{5694CD}-0.87 & 0.00 & \cellcolor[HTML]{649DD1}-0.80 & 0.00 & \cellcolor[HTML]{FFFFFD}0.02 & \cellcolor[HTML]{CCCCCC}0.90 \\
\bottomrule
\end{tabular}

==> tables/corr-ttr.tex <==
\begin{tabular}{@{}l@{\hspace{2mm}}l
S[table-format=+1.2]S[table-format=1.2]
S[table-format=+1.2]S[table-format=1.2]
S[table-format=+1.2]S[table-format=1.2]@{}
}
\toprule
\textbf{Src} & \textbf{Target} & \multicolumn{2}{c}{\textbf{Monoling.}} & \multicolumn{2}{c}{\textbf{mBERT}} & \multicolumn{2}{c}{\textbf{XLM-R}} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}
 &  & \multicolumn{1}{c}{$\rho$} & \multicolumn{1}{c}{p} & \multicolumn{1}{c}{$\rho$} & \multicolumn{1}{c}{p} & \multicolumn{1}{c}{$\rho$} & \multicolumn{1}{c}{p} \\
 \midrule
Ger. & Als. G. & \cellcolor[HTML]{FFEBAF}0.79 & 0.00 & \cellcolor[HTML]{FFF6DA}0.37 & 0.05 & \cellcolor[HTML]{FFF2C9}0.53 & 0.00 \\
Ger. & Swiss G. & \cellcolor[HTML]{FFF5D5}0.42 & 0.02 & \cellcolor[HTML]{FFFDF4}0.11 & \cellcolor[HTML]{CCCCCC}0.57 & \cellcolor[HTML]{FFFAEA}0.21 & \cellcolor[HTML]{CCCCCC}0.26 \\
Ger. & L. Saxon & \cellcolor[HTML]{FFE7A1}0.93 & 0.00 & \cellcolor[HTML]{FFEFC1}0.62 & 0.00 & \cellcolor[HTML]{FFEDB9}0.69 & 0.00 \\
Dutch & L. Saxon & \cellcolor[HTML]{FFF2C9}0.53 & 0.00 & \cellcolor[HTML]{9DC1E2}-0.50 & 0.00 & \cellcolor[HTML]{FFFCF1}0.15 & \cellcolor[HTML]{CCCCCC}0.44 \\
Bokm. & East N. & \cellcolor[HTML]{FFFBF0}0.16 & \cellcolor[HTML]{CCCCCC}0.41 & \cellcolor[HTML]{649DD1}-0.80 & 0.00 & \cellcolor[HTML]{9FC3E2}-0.49 & 0.01 \\
Bokm. & North N. & \cellcolor[HTML]{FFFCF0}0.15 & \cellcolor[HTML]{CCCCCC}0.44 & \cellcolor[HTML]{7CADD8}-0.67 & 0.00 & \cellcolor[HTML]{A7C7E5}-0.45 & 0.01 \\
Bokm. & West N. & \cellcolor[HTML]{FFFCF2}0.13 & \cellcolor[HTML]{CCCCCC}0.49 & \cellcolor[HTML]{70A5D5}-0.73 & 0.00 & \cellcolor[HTML]{92BADF}-0.56 & 0.00 \\
Nynor. & East N. & \cellcolor[HTML]{5D99CF}-0.83 & 0.00 & \cellcolor[HTML]{81B0DA}-0.65 & 0.00 & \cellcolor[HTML]{ECF3F9}-0.10 & \cellcolor[HTML]{CCCCCC}0.62 \\
Nynor. & North N. & \cellcolor[HTML]{5997CE}-0.85 & 0.00 & \cellcolor[HTML]{A4C6E4}-0.47 & 0.01 & \cellcolor[HTML]{F5F9FC}-0.05 & \cellcolor[HTML]{CCCCCC}0.80 \\
Nynor. & West N. & \cellcolor[HTML]{4D8FCA}-0.92 & 0.00 & \cellcolor[HTML]{89B5DC}-0.61 & 0.00 & \cellcolor[HTML]{F2F7FB}-0.06 & \cellcolor[HTML]{CCCCCC}0.74 \\
French & Picard & \cellcolor[HTML]{E3EDF6}-0.14 & \cellcolor[HTML]{CCCCCC}0.45 & \cellcolor[HTML]{FFFBF0}0.15 & \cellcolor[HTML]{CCCCCC}0.42 & \cellcolor[HTML]{FFF7DE}0.33 & \cellcolor[HTML]{CCCCCC}0.07 \\
French & Occitan & \cellcolor[HTML]{FFF4D2}0.45 & 0.01 & \cellcolor[HTML]{5D99CF}-0.83 & 0.00 & \cellcolor[HTML]{FFF5D8}0.39 & 0.03 \\
Spa. & Occitan & \cellcolor[HTML]{FFF6DB}0.36 & \cellcolor[HTML]{CCCCCC}0.05 & \cellcolor[HTML]{458AC8}-0.95 & 0.00 & \cellcolor[HTML]{B0CDE7}-0.41 & 0.03 \\
MSA & Egy. A. & \cellcolor[HTML]{B5D0E9}-0.38 & 0.04 & \cellcolor[HTML]{68A0D2}-0.77 & 0.00 & \cellcolor[HTML]{609BD0}-0.82 & 0.00 \\
MSA & Gulf A. & \cellcolor[HTML]{B8D2EA}-0.37 & 0.05 & \cellcolor[HTML]{468BC8}-0.95 & 0.00 & \cellcolor[HTML]{5E9ACF}-0.83 & 0.00 \\
MSA & Lev. A. & \cellcolor[HTML]{C3D9ED}-0.31 & \cellcolor[HTML]{CCCCCC}0.10 & \cellcolor[HTML]{4E90CB}-0.91 & 0.00 & \cellcolor[HTML]{6FA4D4}-0.74 & 0.00 \\
MSA & Mag. A. & \cellcolor[HTML]{84B1DA}-0.63 & 0.00 & \cellcolor[HTML]{5694CD}-0.87 & 0.00 & \cellcolor[HTML]{95BCDF}-0.54 & 0.00 \\
Fin. & Ost. F. & \cellcolor[HTML]{FFE9A7}0.87 & 0.00 & \cellcolor[HTML]{FFECB3}0.75 & 0.00 & \cellcolor[HTML]{FFFFFC}0.03 & \cellcolor[HTML]{CCCCCC}0.87 \\
Fin. & SE F. & \cellcolor[HTML]{FFE9A6}0.87 & 0.00 & \cellcolor[HTML]{FFECB2}0.76 & 0.00 & \cellcolor[HTML]{FFFBEF}0.17 & \cellcolor[HTML]{CCCCCC}0.38 \\
Fin. & SW F. & \cellcolor[HTML]{FFEBAD}0.81 & 0.00 & \cellcolor[HTML]{FFEDB7}0.71 & 0.00 & \cellcolor[HTML]{FFFEF8}0.08 & \cellcolor[HTML]{CCCCCC}0.69 \\
Fin. & SW tr. & \cellcolor[HTML]{FFEAAD}0.81 & 0.00 & \cellcolor[HTML]{FFEDB9}0.69 & 0.00 & \cellcolor[HTML]{FFFDF5}0.10 & \cellcolor[HTML]{CCCCCC}0.60 \\
Fin. & Sav. F. & \cellcolor[HTML]{FFE9A7}0.87 & 0.00 & \cellcolor[HTML]{FFECB1}0.77 & 0.00 & \cellcolor[HTML]{FFFDF6}0.09 & \cellcolor[HTML]{CCCCCC}0.63 \\
Fin. & Tav. F. & \cellcolor[HTML]{FFE9A7}0.87 & 0.00 & \cellcolor[HTML]{FFEBAE}0.80 & 0.00 & \cellcolor[HTML]{FAFCFD}-0.02 & \cellcolor[HTML]{CCCCCC}0.90 \\\bottomrule
\end{tabular}

==> tables/correlations.tex <==
\begin{tabular}{@{}l@{\hspace{2mm}}l
S[table-format=+1.2]S[table-format=1.2]
S[table-format=+1.2]S[table-format=1.2]
S[table-format=+1.2]S[table-format=1.2]@{}
}
\toprule
\textbf{Src} & \textbf{Target} & \multicolumn{2}{c}{\textbf{Monoling.}} & \multicolumn{2}{c}{\textbf{mBERT}} & \multicolumn{2}{c}{\textbf{XLM-R}} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}
 &  & \multicolumn{1}{c}{$\rho$} & \multicolumn{1}{c}{p} & \multicolumn{1}{c}{$\rho$} & \multicolumn{1}{c}{p} & \multicolumn{1}{c}{$\rho$} & \multicolumn{1}{c}{p} \\
 \midrule
Ger. & Als. G. & \cellcolor[HTML]{5B98CE}\color{white} -0.84 & 0.00 & \cellcolor[HTML]{8DB7DD}-0.58 & 0.00 & \cellcolor[HTML]{7BACD8}\color{white} -0.68 & 0.00 \\
Ger. & Swiss G. & \cellcolor[HTML]{609BD0}\color{white} -0.82 & 0.00 & \cellcolor[HTML]{6FA4D4}\color{white} -0.74 & 0.00 & \cellcolor[HTML]{C3D9ED}-0.31 & \cellcolor[HTML]{CCCCCC}0.10 \\
\textit{Ger.} & \textit{German} & \cellcolor[HTML]{78AAD7}\color{white} -0.69 & 0.00 & \cellcolor[HTML]{6FA5D4}\color{white} -0.74 & 0.00 & \cellcolor[HTML]{77A9D7}\color{white} -0.70 & 0.00 \\
Ger. & L. Saxon & \cellcolor[HTML]{6DA3D4}\color{white} -0.75 & 0.00 & \cellcolor[HTML]{FFF6DA}0.37 & \cellcolor[HTML]{CCCCCC}0.05 & \cellcolor[HTML]{FFF4D3}0.44 & 0.02 \\
Dutch & L. Saxon & \cellcolor[HTML]{5B98CE}\color{white} -0.84 & 0.00 & \cellcolor[HTML]{75A8D6}\color{white} -0.71 & 0.00 & \cellcolor[HTML]{9EC2E2}-0.50 & 0.01 \\
\textit{Dutch} & \textit{Dutch} & \cellcolor[HTML]{5192CC}\color{white} -0.89 & 0.00 & \cellcolor[HTML]{5594CD}\color{white} -0.88 & 0.00 & \cellcolor[HTML]{4D8FCA}\color{white} -0.91 & 0.00 \\
Bokm. & East N. & \cellcolor[HTML]{72A6D5}\color{white} -0.72 & 0.00 & \cellcolor[HTML]{6DA3D4}\color{white} -0.75 & 0.00 & \cellcolor[HTML]{86B3DB}-0.62 & 0.00 \\
Bokm. & North N. & \cellcolor[HTML]{78AAD7}\color{white} -0.69 & 0.00 & \cellcolor[HTML]{76A9D6}\color{white} -0.70 & 0.00 & \cellcolor[HTML]{7AABD8}\color{white} -0.68 & 0.00 \\
Bokm. & West N. & \cellcolor[HTML]{6DA3D4}\color{white} -0.75 & 0.00 & \cellcolor[HTML]{5997CE}\color{white} -0.85 & 0.00 & \cellcolor[HTML]{73A7D5}\color{white} -0.72 & 0.00 \\
Nynor. & East N. & \cellcolor[HTML]{77A9D7}\color{white} -0.70 & 0.00 & \cellcolor[HTML]{5393CC}\color{white} -0.88 & 0.00 & \cellcolor[HTML]{478BC9}\color{white} -0.94 & 0.00 \\
Nynor. & North N. & \cellcolor[HTML]{7BACD8}\color{white} -0.68 & 0.00 & \cellcolor[HTML]{659ED1}\color{white} -0.79 & 0.00 & \cellcolor[HTML]{498CC9}\color{white} -0.94 & 0.00 \\
Nynor. & West N. & \cellcolor[HTML]{83B1DA}-0.64 & 0.00 & \cellcolor[HTML]{5997CE}\color{white} -0.85 & 0.00 & \cellcolor[HTML]{478BC9}\color{white} -0.95 & 0.00 \\
\textit{Bokm.} & \textit{Bokm.} & \cellcolor[HTML]{468BC8}\color{white} -0.95 & 0.00 & \cellcolor[HTML]{4489C8}\color{white} -0.96 & 0.00 & \cellcolor[HTML]{4489C8}\color{white} -0.96 & 0.00 \\
\textit{Nynor.} & \textit{Nynor.} & \cellcolor[HTML]{4389C7}\color{white} -0.97 & 0.00 & \cellcolor[HTML]{4187C7}\color{white} -0.98 & 0.00 & \cellcolor[HTML]{4187C7}\color{white} -0.98 & 0.00 \\
French & Picard & \cellcolor[HTML]{A7C7E5}-0.45 & 0.01 & \cellcolor[HTML]{609BD0}\color{white} -0.82 & 0.00 & \cellcolor[HTML]{5795CD}\color{white} -0.86 & 0.00 \\
\textit{French} & \textit{French} & \cellcolor[HTML]{3F86C6}\color{white} -0.99 & 0.00 & \cellcolor[HTML]{5091CB}\color{white} -0.90 & 0.00 & \cellcolor[HTML]{4389C7}\color{white} -0.97 & 0.00 \\
French & Occitan & \cellcolor[HTML]{6CA2D3}\color{white} -0.76 & 0.00 & \cellcolor[HTML]{A7C7E5}-0.45 & 0.01 & \cellcolor[HTML]{B1CEE8}-0.40 & 0.03 \\
Spa. & Occitan & \cellcolor[HTML]{82B0DA}-0.64 & 0.00 & \cellcolor[HTML]{B5D0E9}-0.38 & 0.04 & \cellcolor[HTML]{75A8D6}\color{white} -0.71 & 0.00 \\
\textit{Spa.} & \textit{Spanish} & \cellcolor[HTML]{478BC8}\color{white} -0.95 & 0.00 & \cellcolor[HTML]{458AC8}\color{white} -0.95 & 0.00 & \cellcolor[HTML]{4388C7}\color{white} -0.97 & 0.00 \\
MSA & Egy. A. & \cellcolor[HTML]{5493CC}\color{white} -0.88 & 0.00 & \cellcolor[HTML]{4F90CB}\color{white} -0.91 & 0.00 & \cellcolor[HTML]{5090CB}\color{white} -0.90 & 0.00 \\
MSA & Gulf A. & \cellcolor[HTML]{5292CC}\color{white} -0.89 & 0.00 & \cellcolor[HTML]{478BC8}\color{white} -0.95 & 0.00 & \cellcolor[HTML]{5191CC}\color{white} -0.89 & 0.00 \\
MSA & Lev. A. & \cellcolor[HTML]{4F90CB}\color{white} -0.91 & 0.00 & \cellcolor[HTML]{5594CD}\color{white} -0.87 & 0.00 & \cellcolor[HTML]{5E9ACF}\color{white} -0.83 & 0.00 \\
MSA & Mag. A. & \cellcolor[HTML]{74A7D6}\color{white} -0.72 & 0.00 & \cellcolor[HTML]{77A9D7}\color{white} -0.70 & 0.00 & \cellcolor[HTML]{609BD0}\color{white} -0.82 & 0.00 \\
\textit{MSA} & \textit{MSA} & \cellcolor[HTML]{4489C8}\color{white} -0.96 & 0.00 & \cellcolor[HTML]{458AC8}\color{white} -0.96 & 0.00 & \cellcolor[HTML]{4489C8}\color{white} -0.96 & 0.00 \\
Fin. & Ost. F. & \cellcolor[HTML]{A5C6E4}-0.46 & 0.01 & \cellcolor[HTML]{5090CB}\color{white} -0.90 & 0.00 & \cellcolor[HTML]{FFF8E1}0.30 & \cellcolor[HTML]{CCCCCC}0.11 \\
Fin. & SE F. & \cellcolor[HTML]{75A8D6}\color{white} -0.71 & 0.00 & \cellcolor[HTML]{4A8DC9}\color{white} -0.93 & 0.00 & \cellcolor[HTML]{FFFAEA}0.21 & \cellcolor[HTML]{CCCCCC}0.27 \\
Fin. & SW F. & \cellcolor[HTML]{EDF3F9}-0.09 & \cellcolor[HTML]{CCCCCC}0.63 & \cellcolor[HTML]{488CC9}\color{white} -0.94 & 0.00 & \cellcolor[HTML]{FFF8E2}0.29 & \cellcolor[HTML]{CCCCCC}0.12 \\
Fin. & SW tr. & \cellcolor[HTML]{B1CEE8}-0.40 & 0.03 & \cellcolor[HTML]{498CC9}\color{white} -0.94 & 0.00 & \cellcolor[HTML]{FFF9E4}0.27 & \cellcolor[HTML]{CCCCCC}0.15 \\
Fin. & Sav. F. & \cellcolor[HTML]{7AABD8}\color{white} -0.68 & 0.00 & \cellcolor[HTML]{5292CC}\color{white} -0.89 & 0.00 & \cellcolor[HTML]{FFF9E7}0.24 & \cellcolor[HTML]{CCCCCC}0.20 \\
Fin. & Tav. F. & \cellcolor[HTML]{74A8D6}\color{white} -0.71 & 0.00 & \cellcolor[HTML]{5292CC}\color{white} -0.89 & 0.00 & \cellcolor[HTML]{FFF7DD}0.34 & \cellcolor[HTML]{CCCCCC}0.07 \\
\textit{Fin.} & \textit{Finnish} & \cellcolor[HTML]{478BC9}\color{white} -0.95 & 0.00 & \cellcolor[HTML]{4489C8}\color{white} -0.96 & 0.00 & \cellcolor[HTML]{4489C8}\color{white} -0.96 & 0.00 \\
\bottomrule
\end{tabular}
